Descriptive Kernel Convolution Network with Improved Random Walk Kernel

Graph kernels used to be the dominant approach to feature engineering for structured data, which are superseded by modern GNNs as the former lacks learnability. Recently, a suite of Kernel Convolution Networks (KCNs) successfully revitalized graph kernels by introducing learnability, which convolves input with learnable hidden graphs using a certain graph kernel. The random walk kernel (RWK) has been used as the default kernel in many KCNs, gaining increasing attention. In this paper, we first revisit the RWK and its current usage in KCNs, revealing several shortcomings of the existing designs, and propose an improved graph kernel RWK+, by introducing color-matching random walks and deriving its efficient computation. We then propose RWK+CN, a KCN that uses RWK+ as the core kernel to learn descriptive graph features with an unsupervised objective, which can not be achieved by GNNs. Further, by unrolling RWK+, we discover its connection with a regular GCN layer, and propose a novel GNN layer RWK+Conv. In the first part of experiments, we demonstrate the descriptive learning ability of RWK+CN with the improved random walk kernel RWK+ on unsupervised pattern mining tasks; in the second part, we show the effectiveness of RWK+ for a variety of KCN architectures and supervised graph learning tasks, and demonstrate the expressiveness of RWK+Conv layer, especially on the graph-level tasks. RWK+ and RWK+Conv adapt to various real-world applications, including web applications such as bot detection in a web-scale Twitter social network, and community classification in Reddit social interaction networks.

==> 031method-init.tex <==

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AUTHOR: Christos Faloutsos
% INSTITUTION: CMU
% DATE: April 2019
% GOAL: to streamline the paper presentations
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we firstly investigate random walk kernels (\rwk) that used in the previous works with an unsupervised objective.
Next, we show how we can improve it by matching the labels on every intermediate node in a path, which we call \colormatch.
To justify its importance, we conduct experiments on pattern mining and demonstrate our improvement from original \rwk.
\leman{make sure you dedicate subsections to every improvement: 1. color matching and its scalable re-formulation (Lingxiao's gems from yesterday), 2. ``structural colors'', 3. diversity regularization toward distinctive pattern mining. i am writing them in the intro in that order.}


\subsection{Random Walk Kernels (\rwk)}

\paragraph{Unlabeled Case}
Given a undirected graph $G=(V, E)$, its product graph with another graph $G^{\prime}=(V^{\prime}, E^{\prime})$ can be defined as $G_{\times}=(V_{\times}, E_{\times})$, where $V$ and $E$ denote the node and edge sets, respectively.

Given a graph database $\mathcal{A}$, where $\boldsymbol{A}_{n \times n} \in \mathcal{A}$ is the adjacency matrix of a graph, and a graph kernel $\boldsymbol{B}_{m \times m}$, the random walk kernel (RWK) similarity with unweighted steps $k$ is defined as follows:
\begin{equation}
\begin{split}
r^{(k)}(\mathcal{A}, \boldsymbol{B}) & 
= \sum_{\boldsymbol{A} \in \mathcal{A}} {\sum_{i=1}^{nm}\sum_{j=1}^{nm} {
\begin{bmatrix}
(\boldsymbol{A} \otimes \boldsymbol{B})^{k}
\end{bmatrix}_{ij}
}
}
\\
& = 
(\sum_{i=1}^{nm}\sum_{j=1}^{nm}
\begin{bmatrix}
\sum_{\boldsymbol{A} \in \mathcal{A}}
{\boldsymbol{A}^{k}}
\end{bmatrix}_{ij})
\cdot
(\sum_{i=1}^{nm}\sum_{j=1}^{nm}
\begin{bmatrix}
\boldsymbol{B}^{k}
\end{bmatrix}_{ij})
\end{split}
\end{equation}
Given an optimization task where $\mathcal{A}$ is fixed, if our goal is to maximize the RWK similarity and learn the structure of $\boldsymbol{B}$, then $\boldsymbol{B}^{k}$ with more edges is always preferred.
In other words, this optimization only cares about how many edges $\boldsymbol{B}^{k}$ has, ignoring all the information from $\mathcal{A}$.

If further the set of node features $\mathcal{X}$ is given, where $\boldsymbol{X}_{n \times f} \in \mathcal{X}$ are the node features of the graph in $\mathcal{A}$, and the node features $\boldsymbol{Z}_{m \times f}$ of the graph kernel are given as well, the random walk kernel (RWK) similarity is defined as follows:
\begin{equation}
\begin{split}
r^{(k)}(\mathcal{A}, \boldsymbol{B}) & 
= \sum_{\boldsymbol{A} \in \mathcal{A}} {\sum_{i=1}^{nm}\sum_{j=1}^{nm} {
\begin{bmatrix}
(\boldsymbol{s}\boldsymbol{s}^{\top}) \odot (\boldsymbol{A} \otimes \boldsymbol{B})^{k}
\end{bmatrix}_{ij}
}
}
\\
& = \sum_{i=1}^{f}\sum_{j=1}^{f}
\begin{bmatrix}
(\sum_{\boldsymbol{A} \in \mathcal{A}, \boldsymbol{X} \in \mathcal{X}}
{\boldsymbol{X}^{\top}\boldsymbol{A}^{k} \boldsymbol{X}}) 
\odot
(\boldsymbol{Z}^{\top}\boldsymbol{B}^{k}\boldsymbol{Z}) 
\end{bmatrix}_{ij},
\end{split}
\end{equation}
where $\boldsymbol{s}_{nm \times 1} = \text{vec}(\boldsymbol{Z} \boldsymbol{X}^{\top})$.

To prevent the similarity from exploding after walking $k$ steps, we degree-normalize the adjacency matrix before walking. The degree-normalized function is:
\begin{equation}
d(A) = \boldsymbol{D}^{-\frac{1}{2}} \boldsymbol{A} \boldsymbol{D}^{-\frac{1}{2}},
\end{equation}
where $\boldsymbol{D}$ is the degree matrix of an adjacency matrix $\boldsymbol{A}$.
The optimization problem of maximizing RWK similarity is formulated as follows:
\begin{equation}
\max_{\boldsymbol{B}, \boldsymbol{Z}} 
\sum_{i=1}^{f}\sum_{j=1}^{f}
\begin{bmatrix}
(\sum_{\boldsymbol{A} \in \mathcal{A}, \boldsymbol{X} \in \mathcal{X}}
{\boldsymbol{X}^{\top}d(\boldsymbol{A})^{k} \boldsymbol{X}}) 
\odot
(\boldsymbol{Z}^{\top}d(\boldsymbol{B})^{k}\boldsymbol{Z}) 
\end{bmatrix}_{ij},
\end{equation}

$\boldsymbol{s}$ can be thought as the flattened feature similarities between nodes in $\boldsymbol{A}$ and $\boldsymbol{B}$:
\begin{equation}
\boldsymbol{s} = 
\begin{bmatrix}
\langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{1}\rangle \\ 
\langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{2}\rangle \\
\cdots \\ 
\langle\boldsymbol{X}_{2}, \boldsymbol{Z}_{1}\rangle \\
\langle\boldsymbol{X}_{2}, \boldsymbol{Z}_{2}\rangle \\
\cdots \\ 
\langle\boldsymbol{X}_{n}, \boldsymbol{Z}_{m}\rangle 
\end{bmatrix},
\end{equation}
where $\boldsymbol{X}_{i}$ denotes the $i$-th row of $\boldsymbol{X}$, and $\langle \cdot, \cdot \rangle$ denotes the inner product.
$\boldsymbol{s}\boldsymbol{s}^{\top}$ can then be thought as the feature similarities between super-nodes in $\boldsymbol{A} \otimes \boldsymbol{B}$:
% \begin{equation}
% \boldsymbol{s}\boldsymbol{s}^{\top} = 
% \begin{bmatrix}
% \langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{1}\rangle \cdot \langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{1}\rangle & \dotsb &
% \langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{1}\rangle \cdot \langle \boldsymbol{X}_{2}, \boldsymbol{Z}_{1}\rangle & \dotsb &
% \langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{1}\rangle \cdot \langle \boldsymbol{X}_{n}, \boldsymbol{Z}_{m}\rangle \\ 
% \langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{2}\rangle \cdot \langle \boldsymbol{X}_{1}, \boldsymbol{Z}_{1}\rangle & \dotsb &
% \langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{2}\rangle \cdot \langle \boldsymbol{X}_{2}, \boldsymbol{Z}_{1}\rangle & \dotsb &
% \langle\boldsymbol{X}_{1}, \boldsymbol{Z}_{2}\rangle \cdot \langle \boldsymbol{X}_{n}, \boldsymbol{Z}_{m}\rangle \\ 
% \vdots & \dotsb &
% \ddots & \dotsb & \vdots \\ 
% \langle\boldsymbol{X}_{n}, \boldsymbol{Z}_{m}\rangle \cdot \langle \boldsymbol{X}_{1}, \boldsymbol{Z}_{1}\rangle & \dotsb &
% \langle\boldsymbol{X}_{n}, \boldsymbol{Z}_{m}\rangle \cdot \langle \boldsymbol{X}_{2}, \boldsymbol{Z}_{1}\rangle & \dotsb &
% \langle\boldsymbol{X}_{n}, \boldsymbol{Z}_{m}\rangle \cdot \langle \boldsymbol{X}_{n}, \boldsymbol{Z}_{m}\rangle \\ 
% \end{bmatrix}
% \end{equation}

RWK similarity identifies a path $((i_{1}, j_{1}), \dots, (i_{k}, j_{k}))$ on $\boldsymbol{A} \otimes \boldsymbol{B}$ to be valid if $\boldsymbol{X}_{i_{1}}$ and $\boldsymbol{X}_{i_{k}}$ are similar to $\boldsymbol{Z}_{j_{1}}$ and $\boldsymbol{Z}_{j_{k}}$ (only the beginning and the ending pairs), respectively.

To walk more accurately, all steps in a path need to be valid. In other words, for a path $((i_{1}, j_{1}), \dots, (i_{k}, j_{k}))$, $\boldsymbol{X}_{i_{1}}, \dots, \boldsymbol{X}_{i_{k}}$ needs to be similar to $\boldsymbol{Z}_{j_{1}}, \dots, \boldsymbol{Z}_{j_{k}}$ ($k$ pairs), respectively. 
This can also be thought of as color-matching (CM).

Thus, CM-RWK similarity can be defined as:
\begin{equation}
r^{*(k)}(\mathcal{A}, \boldsymbol{B})
= \sum_{\boldsymbol{A} \in \mathcal{A}} {\sum_{i=1}^{nm}\sum_{j=1}^{nm} {
\begin{bmatrix}
((\boldsymbol{s}\boldsymbol{s}^{\top}) \odot (\boldsymbol{A} \otimes \boldsymbol{B}))^{k}
\end{bmatrix}_{ij}
}}
\end{equation}

To motivate the kernel to learn meaningful structure, when optimizing, we degree-normalize the kernel.
This makes each row (or column) of the kernel sum into a value close to one.
Thus, only those essential edges that contribute the most to the similarity are kept.
The optimization problem of maximizing CM-RWK similarity is then formulated as follows:
\begin{equation}
\max_{\boldsymbol{B}, \boldsymbol{Z}} \sum_{\boldsymbol{A} \in \mathcal{A}} {\sum_{i=1}^{nm}\sum_{j=1}^{nm} {
\begin{bmatrix}
((\boldsymbol{s}\boldsymbol{s}^{\top}) \odot (\boldsymbol{A} \otimes d(\boldsymbol{B})))^{k}
\end{bmatrix}_{ij}
}}
\end{equation}

==> makefile <==
####################################
# Author: Christos Faloutsos
# Date: March 2018
####################################

MAIN= paper
FINAL= final
SAVE-DIR=SAVE
TEXPARTS= \
    000abstract.tex \
    010introduction.tex \
    020background.tex \
    030method.tex \
    040experiment.tex \
    060conclusion.tex \
    070appendix.tex \
    080listOfToDo.tex \
    dfn.tex

BIBPARTS= BIB/*.bib BIB/catbib.bash
FIGPARTS= FIG/*.png FIG-TIKZ/*.tex
STYPARTS= sig-alternate.cls
OTHER= mkfinal.pl makefile README.txt
ALL= $(MAIN).tex $(TEXPARTS) $(BIBPARTS) $(FIGPARTS) $(STYPARTS) $(OTHER)

$(MAIN).pdf: $(MAIN).tex $(TEXPARTS) 
	pdflatex $(MAIN).tex
	bibtex $(MAIN)
	pdflatex $(MAIN).tex
	pdflatex $(MAIN).tex

final: $(FINAL).pdf

$(FINAL).pdf: $(MAIN).tex mkfinal.pl
	perl mkfinal.pl $(MAIN).tex > $(FINAL).tex
	pdflatex $(FINAL).tex
	bibtex $(FINAL)
	pdflatex $(FINAL).tex
	pdflatex $(FINAL).tex

try: $(MAIN).tex
	pdflatex $(MAIN)


clean:
	\rm -f *.dvi $(MAIN).ps *.bbl *.aux *.log *.blg *.toc all.tar* uu \
	*~ *.bak *.lbl *.brf $(MAIN).synctex.gz \
	*.out *.soc *.tdo *.loc

spotless: clean
	\rm -f $(MAIN).ps $(MAIN).pdf
	\rm -f $(FINAL).*
	\rm -rf TST

all.tar:
	tar cvfh all.tar $(ALL)

save: all.tar
	mv all.tar $(SAVE-DIR)

